Generalized Category Discovery with Clustering Assignment Consistency

Generalized category discovery (GCD) is a recently proposed open-world task. Given a set of images consisting of labeled and unlabeled instances, the goal of GCD is to automatically cluster the unlabeled samples using information transferred from the labeled dataset. The unlabeled dataset comprises both known and novel classes. The main challenge is that unlabeled novel class samples and unlabeled known class samples are mixed together in the unlabeled dataset. To address the GCD without knowing the class number of unlabeled dataset, we propose a co-training-based framework that encourages clustering consistency. Specifically, we first introduce weak and strong augmentation transformations to generate two sufficiently different views for the same sample. Then, based on the co-training assumption, we propose a consistency representation learning strategy, which encourages consistency between feature-prototype similarity and clustering assignment. Finally, we use the discriminative embeddings learned from the semi-supervised representation learning process to construct an original sparse network and use a community detection method to obtain the clustering results and the number of categories simultaneously. Extensive experiments show that our method achieves state-of-the-art performance on three generic benchmarks and three fine-grained visual recognition datasets. Especially in the ImageNet-100 data set, our method significantly exceeds the best baseline by 15.5\% and 7.0\% on the \texttt{Novel} and \texttt{All} classes, respectively.

==> figures/t-sne.tex <==
\begin{figure}[ht]
	\begin{minipage}{0.32\linewidth}
		\vspace{3pt}
		\centerline{\includegraphics[width=\textwidth,trim=50 50 50 50,clip]{figures/cifar10_dino.eps}}
		\centerline{(a) DINO}
	\end{minipage}
	\begin{minipage}{0.32\linewidth}
		\vspace{3pt}
		\centerline{\includegraphics[width=\textwidth, trim=50 50 50 50,clip]{figures/cifar10_gcd.eps}}
		\centerline{(b) GCD}
	\end{minipage}
	\begin{minipage}{0.32\linewidth}
		\vspace{3pt}
		\centerline{\includegraphics[width=\textwidth,trim=50 50 50 50,clip]{figures/cifar10_ours.eps}}
		\centerline{(c) Ours}
	\end{minipage}
	\caption{T-SNE visualization of the embeddings on CIFAR-10. The embedding clustering shows that our proposed method encourages the expansion of the distance between different clusters.}
	\label{fig:t-sne}
\end{figure}

==> tables/strong_aug.tex <==
\begin{wrapfigure}{r}{6cm}
		\centering
		\caption{List of strong augmentations for images.}
		\label{tab:strong_aug}
		\begin{tabular}{c|c}
			\toprule
			\textbf{Transformations} & \textbf{Mag Range} \\
			\midrule
			Shear X, Y & [-0.3, 0.3] \\
			\hline
			Translate X, Y & [-0.3, 0.3] \\
			\hline
			Roate & [-30, 30] \\
			\hline
			AutoContrast & 0 or 1 \\
			\hline
			Invert & 0 or 1 \\
			\hline
			Equalize & 0 or 1
			\\
			\hline
			Solarize & [0, 256] \\
			\hline
			Posterize & [4, 8] \\
			\hline
			Contrast & [0.05, 0.95] \\
			\hline
			Color & [0.05, 0.95] \\
			\hline
			Brightness & [0.05, 0.95] \\
			\hline
			Sharpeness & [0.05, 0.95] \\
			\bottomrule
		\end{tabular}
\end{wrapfigure}

